CoBa: Convergence Balancer for Multitask Finetuning of Large Language Models

Multi-task learning (MTL) benefits the fine-tuning of large language models (LLMs) by providing a single model with improved performance and generalization ability across tasks, presenting a resource-efficient alternative to developing separate models for each task. Yet, existing MTL strategies for LLMs often fall short by either being computationally intensive or failing to ensure simultaneous task convergence. This paper presents CoBa, a new MTL approach designed to effectively manage task convergence balance with minimal computational overhead. Utilizing Relative Convergence Scores (RCS), Absolute Convergence Scores (ACS), and a Divergence Factor (DF), CoBa dynamically adjusts task weights during the training process, ensuring that the validation loss of all tasks progress towards convergence at an even pace while mitigating the issue of individual task divergence. The results of our experiments involving three disparate datasets underscore that this approach not only fosters equilibrium in task convergence but enhances the LLMs' performance by up to 13% relative to the second-best baselines. Code is open-sourced at https://github.com/codefuse-ai/MFTCoder.

==> contents/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we propose CoBa, a novel MTL method for LLMs that simultaneously achieves convergence balance with low computational complexity. Extensive experiments on three real-world datasets have demonstrated the efficacy and efficiency of the proposed method.

==> contents/experiment.tex <==
\section{Experiments}
\label{sec:experiment}

In this section, we assess the performance of the CoBa across three diverse datasets: the \textbf{Code Completion (CC) Dataset}, encompassing five programming languages; the \textbf{Code-Related Task (CRT) Dataset}, featuring five unique programming tasks; and \textbf{XTREME-UP}, which delves into question-answering across nine natural languages. The tasks within these datasets are inherently related and generative, making them ideal candidates for MTL experiments on LLM. For further insights into the datasets, readers are directed to the Appendix~\ref{app:datasets}.

Our evaluation benchmarks the CoBa against 8 state-of-the-art (SOTA) baselines\footnote{We exclude MetaWeighting due to its high computational demands, as detailed in Table~\ref{tab:time-complexity}, thereby rendering it prohibitive for use with LLMs.}: \textbf{Single-Task Learning (STL)}, which finetunes each task in isolation; \textbf{Uniform}~\cite{liu2023mftcoder}, applying equal weights to all tasks in a MTL framework; \textbf{GradNorm}~\cite{chen2018gradnorm}, a method that optimizes the task weights iteratively such that task-specific gradients are of similar magnitude; \textbf{LBTW}~\cite{liu2019loss}, which dynamically adjusts task weights according to the ratio of current to initial loss $\omega_i(t) = (\ell_i(t) / \ell_0(t))^b$, parameterized by a hyperparameter $b$; and \textbf{FAMO}~\cite{liu2024famo}, aimed at optimizing weights to enhance the minimal improvement rate across tasks. Notably, the last three methods were originally designed to optimize training loss. In pursuit of enhanced generalization for the fine-tuned models, we have adapted these methods to focus on validation loss, denoted as \textbf{LBTW$^*$}, \textbf{GradNorm$^*$}, and \textbf{FAMO$^*$}. Except for STL and Uniform, all methods strive to balance convergence across tasks, demonstrating their potential to compete with CoBa. The detailed experiment setup is described in the Appendix~\ref{app:setup}.





\begin{table}[t]%\small
    \centering
    %\setlength{\tabcolsep}{12pt}
    \caption{Performance on the CC Dataset with Phi-1.5-1.3B model.}
    \vspace{-1ex}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \pmb{Method} & \pmb{Python} & \pmb{Java} & \pmb{C++} & \pmb{JS} & \pmb{Go} & \pmb{Avg} \\
        \midrule
        STL & 48.8 & 23.8 & 20.7 & 26.8 & 17.1 & 27.4 \\
        Uniform & 48.2 & 22.6 & 23.2 & 27.4 & 16.5 & 27.6 \\
        GradNorm & 47.0 & 22.0 & 23.2 &	26.8 &	16.5 & 27.1 \\
        GradNorm$^{*}$ & 47.6 &	25.6 &	22.0 & 26.2 & 17.1 & 27.7 \\
        LBTW & 47.0 & 22.0 & 22.3 & 28.1 & \pmb{18.3} & 27.6 \\
        LBTW$^{*}$ & 48.2 & 23.2 & 23.8 & 26.8 & \pmb{18.3} & 28.1 \\
        FAMO & 48.2 & \pmb{26.2} & 21.3 &	26.2 &	17.1 & 27.8 \\
        FAMO$^{*}$ & 48.2 & 23.2 & \pmb{25.6} & 26.8 & 17.7 & 28.3 \\
        CoBa & \pmb{49.4} & 24.4 & 25.0 & \pmb{29.9} & \pmb{18.3} & \pmb{29.4} \\
        \bottomrule
    \end{tabular}}
    \label{tab:5languages-phi-result}
    \vspace{-3ex}
\end{table}









\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.8\textwidth]{images/3tasks_f1.pdf}
    \vspace{-2ex}
    \caption{Experimental results on XTREME-UP dataset with 3-tasks setting.}
    \label{fig:xtreme-up-3tasks}
    \vspace{-3ex}
\end{figure*}





\begin{comment}
    \subsection{Baselines}
We compare our method with:

\textbf{Single-Task Learning (STL):} learning each task independently.

\textbf{Uniform:} learning tasks simultaneously using uniform task weights, and the implementation refers to MFTCoder~\cite{liu2023mftcoder}.

\textbf{GradNorm:} learning tasks simultaneously using gradient normalization method~\cite{chen2018gradnorm}. \textbf{GradNorm$^{*}$} is an enhanced version that updates weights using the gradient normalization method applied to validation dataset.

\textbf{LBTW:} learning tasks simultaneously using Loss Balanced Task Weighting method~\cite{liu2019loss}. \textbf{LBTW$^{*}$} is an enhanced version that allocates weights based on the learning speed computed from validation dataset.

\textbf{FAMO:} learning tasks simultaneously using Fast Adaptive Multitask Optimization method~\cite{liu2024famo}. \textbf{FAMO$^{*}$} is an enhanced version that updates weights using the fast adaptive multitask optimization method applied to validation dataset.

\yh{mention how we choose the basline methods and exclude metaweighting and other methods at the beginning of this subsection.}
MetaWeighting~\cite{mao2022metaweighting} method requires the calculation of gradients for each task within each batch, with the number of forward and backward passes being directly proportional to the number of tasks. This introduces a computational load that is a multiple of the number of tasks, hence we did not replicate the MetaWeighting method.

Due to the large size of the Code-related Task Dataset and the high computational complexity of GradNorm$^{*}$, LBTW$^{*}$ and FAMO$^{*}$, we do not conduct this experiment using these three methods.

\end{comment}




\subsection{Results for CC and CRT}
Table~\ref{tab:5languages-phi-result} shows the Pass@1 metric for all code completion (CC) tasks resulting from all methods. Moreover, Figure~\ref{fig:5languages-loss} graphically presents the normalized loss ratio across all tasks for each method. \textbf{CoBa demonstrates superior performance over the baseline methods in the Pass@1 metric for five programming languages, achieving a minimum of 4\% relative improvement in the average Pass@1 score} (calculated as $(29.4 - 28.3) / 28.3 = 4\%$). In addition, adaptations of FAMO, LBTW, and GradNorm to the validation loss rather than the training loss (i.e., FAMO$^*$, LBTW$^*$, and GradNorm$^*$) show enhanced performance. This enhancement signifies the importance of balancing convergence speed based on validation loss for better generalization, as pointed out in~\cite{mao2022metaweighting}. Indeed, FAMO$^*$ closely trails the performance of CoBa. However, Figure~\ref{fig:5languages-loss} reveals its limitation in preemptively addressing the divergence in the Python completion task, thus limiting its overall efficacy. As an alternative, by utilizing the ACS and DF, CoBa effectively neutralizes the divergence of the Python task. Contrastingly, despite its aims of learning all tasks at an equal pace, GradNorm's performance lags behind counterparts such as CoBa, FAMO, and LBTW. This underperformance may be attributed to GradNorm's strategy of adjusting loss weights using the same learning rate as the model parameters, a tactic that proves ineffective due to the typically small learning rates employed in training LLMs. Consequently, the weights adjusted by GradNorm remain almost identical to the initial uniform weights, failing to dynamically respond to the learning progress and hampering convergence balance. 

Regarding the CRT Dataset, its results are similar to those of the CC dataset, and so we defer its detailed discussion to Appendix~\ref{app:results_code_related}. Notably, in contrast with other state-of-the-art methods, \textbf{CoBa excelled in the Code Completion and Unit Test Generation tasks, recording substantial relative average Pass@1 improvements of at least 6\% and 13\%, respectively.}
%Note that the sample sizes of tasks in this dataset are at least 10 times bigger than those in the first dataset. The high computational complexity of FAMO$^*$ and GradNorm$^*$ leads to a very long processing duration, taking at least four days on 16 A100 GPUs. On the contrary, \textbf{CoBa manages to process the data within two days and still comes out on top, underlining its potential efficacy within large-scale data scenarios}.


%On the other hand, as shown in Figure~\ref{fig:5languages-loss}, our method can effectively prevent divergence in the validation loss for Python and JavaScript languages, ultimately achieving convergence balance. The figure also demonstrates that FAMO has some capability to prevent divergence, but the model converges more slowly, resulting in an evaluation outcome that is not as favorable as our method.



\subsection{Results for XTREME-UP}
In this study, we conduct experiments across three groups, each consisting of 3, 6, and 9 tasks, with a mix of high and low-resource languages. We perform five trials per group to assess the resilience of our proposed method, CoBa, against varying task quantities and its capability to generalize performance for low-resource languages. The results, presented in Figure~\ref{fig:xtreme-up-3tasks} and Figures~\ref{fig:xtreme-up-6tasks} and~\ref{fig:xtreme-up-9tasks} in the appendix, consistently show \textbf{CoBa outperforming all baselines in terms of the average span $F_1$ score across all conditions}. Notably, the effectiveness of CoBa remains stable regardless of the number of tasks, illustrating its adaptability. Importantly, CoBa showcases pronounced enhancements in performance for low-resource languages, like Bengali (bn) and Telugu (te), with a 3\% to 5\% absolute increase in span $F_1$ scores over the Single-Task Learning (STL) approach. This underscores CoBa's proficiency in improving generalization for tasks with limited data availability. For high-resource languages, CoBa's performance matches or surpasses that of STL, suggesting that managing task convergence simultaneously can catalyze synergistic benefits among related tasks. Our experiment also reveals that FAMO generally underperforms, likely due to its sensitivity to the regularization coefficient $\gamma$~\cite{liu2024famo}, which requires manual customization for each dataset. In contrast, FAMO$^*$, which is designed for the validation set, bypasses regularization and shows much better performance.\footnote{The regularization step in FAMO is specifically needed for gradient approximation based on changes in log losses, a process relevant only to its application on the training set. Conversely, FAMO$^*$, which targets the validation set, requires recalculating gradients from scratch. This approach eliminates the need for regularization, leading to more stable performance across various datasets.}


%\yh{Here, we conduct three groups of experiments with respectively 3, 6, and 9 tasks: each group contains a mix of high and low-resource languages, and five trials are run for each to examine the resilience of our proposed method vis-a-vis the number of tasks and test the performance generalization for low-resource languages. The results are depicted in Figure~\ref{fig:xtreme-up-3tasks} as well as Figures~\ref{fig:xtreme-up-6tasks} and~\ref{fig:xtreme-up-9tasks} in the appendix. Once again, CoBa consistently outperforms all baseline methods in terms of the averaged span $F_1$ score across all groups and trials. It is worth noting that \textbf{CoBa's superiority is unaffected by the number of tasks involved in each group of experiments}. More importantly, CoBa demonstrates significant improvements over other methods when tested on low-resource languages, such as Bengali (bn) and Telugu (te). This is evident in the 3\% to 5\% increase in the span $F_1$ score compared to STL which trains each task separately, proving that \textbf{CoBa facilitates better generalization to data-scarce tasks in the MTL scenario}. Meanwhile, CoBa's performance with high-resource languages is either superior or comparable to the STL, implying that simultaneous task convergence can foster mutual enhancement amongst related tasks. Finally, we notice that FAMO generally underperformed on this dataset, a situation likely linked to the sensitivity of its performance to the regularization coefficient $\gamma$, as pointed out in~\cite{liu2024famo}. Ordinarily, $\gamma$ needs manual customization for each dataset; however, all experiments in this paper utilize a constant $\gamma$ value. In contrast, FAMO$^*$ omits this regularization step because it is unnecessary when not approximating the gradient from log loss changes—a process only relevant when FAMO is applied to the training set. Since FAMO$^*$ is designed with the validation set in mind, it necessitates recalculating the gradient from scratch, thereby bypassing the need for regularization and showing much better performance.}


%The three sets of experiments on the XTREME-UP dataset are shown in Figures ~\ref{fig:xtreme-up-3tasks}, ~\ref{fig:xtreme-up-6tasks}, and ~\ref{fig:xtreme-up-9tasks}, where our method outperforms the baseline model in all five rounds of each set, with an average $F_1$ score improvement of over 1\% per group. Notably, for low-resource tasks such as Bengali (bn), Swahili (sw), and Indonesian (id), the multi-task learning approach consistently outperforms single-task learning. Generally, low-resource tasks are more vulnerable to the effects of task imbalance. Due to our method's facilitation of balanced convergence, the gains for low-resource tasks are most pronounced, with nearly 3\% to 5\% increases in $F_1$ score. Moreover, the advantages of our method become increasingly evident as the number of tasks increases. On the other hand, for high-resource tasks such as Arabic (ar) and English (en), our method can match or even surpass the performance of single-task learning. These results reaffirm the importance of convergence balance, enabling our method to achieve the best performance under various task quantities.


\begin{table}[t]%\small
    \centering
    %\setlength{\tabcolsep}{12pt}
    \caption{Ablation study on CC with Phi-1.5-1.3B.}
    \vspace{-1ex}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \pmb{Method} & \pmb{Python} & \pmb{Java} & \pmb{C++} & \pmb{JS} & \pmb{Go} & \pmb{Avg} \\
        \midrule
        CoBa & \pmb{49.4} & 24.4 & \pmb{25.0} & \pmb{29.9} & 18.3 & \pmb{29.4} \\
        \hspace{3mm} w/o RCS & 48.8 & 25.0 & 23.2 & 29.3 & 17.1 & 28.7 \\
        \hspace{3mm} w/o ACS & 47.0 & \pmb{26.8} & 22.6 & 26.8 & 17.1 & 28.1 \\
        \hspace{3mm} $DF \equiv 0.5$ & 47.6 & 23.8 & 23.2 & 26.8 & \pmb{20.1} & 28.3 \\
        \bottomrule
    \end{tabular}}
    \label{tab:5languages-phi-ablation}
    \vspace{-1ex}
\end{table}

\begin{table}[t] %\small
    \centering
    \caption{Performance on the CC Dataset with CodeLlama-13B-Python.}
    \label{tab:5languages-codellama-result}
    \vspace{-1ex}
    %\setlength{\tabcolsep}{12pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \pmb{Method} & \pmb{Python} & \pmb{Java} & \pmb{C++} & \pmb{JS} & \pmb{Go} & \pmb{Avg} \\
        \midrule
        STL & 60.4 & 53.7 & 40.2 & 53.7 & 37.2 & 49.0 \\
        Uniform & 62.2 & 53.1 & 40.8 & 51.8 & 39.6 & 49.5 \\
        GradNorm & 62.8 & 53.1 & 41.5 & 52.4 & 37.2 & 49.4 \\
        GradNorm$^{*}$ & 61.0 & 54.3 & 40.9 & 53.7 & 39.6 & 49.9 \\
        LBTW & 64.0 & 54.9 & 40.8 & 51.8 & 39.0 & 50.1 \\
        LBTW$^{*}$ & 62.2 &	52.4 & \pmb{42.7} & 54.9 & 40.8 & 50.6 \\
        FAMO & 62.2 & 52.4 & 42.1 & 51.8 & 41.5 & 50.0 \\
        FAMO$^{*}$ & 62.2 & 53.1 & 41.5 & 53.1 & 41.5 & 50.2 \\
        CoBa & \pmb{65.9} & \pmb{56.7} & \pmb{42.7} & \pmb{56.7} & \pmb{42.7} & \pmb{52.9} \\
        \bottomrule
    \end{tabular}}
    \vspace{-3ex}
\end{table}

\subsection{Ablation Study and Run Time Analysis}
We first examine \textbf{the impact of RCS, ACS, and DF} within CoBa. The outcomes, cataloged in Table~\ref{tab:5languages-phi-ablation}, reveal a decline in CoBa’s effectiveness when excluding either RCS or ACS, particularly ACS which is crucial for preventing task-specific overfitting. Moreover, a dynamic DF outperforms a fixed one (e.g., constant at 0.5), showcasing the robustness of CoBa's adaptive mechanisms. Figure~\ref{fig:5languages-loss-ablation} further highlights the necessity of combining all three components to ensure that all tasks converge at a similar pace. Next, we evaluate \textbf{CoBa’s adaptability across models of varying sizes} by choosing CodeLlama-13B-Python as the base model. Results in Table~\ref{tab:5languages-codellama-result} highlight CoBa's exceptional performance across all five programming languages, boasting a minimum of a 5\% enhancement in average Pass@1 relative to other SOTA methods. Comparisons between the larger CodeLlama-13B-Python and the smaller Phi-1.5-1.3B models—seen in Table~\ref{tab:5languages-phi-result}—highlighted that larger models boost CoBa's multi-task learning efficacy. This suggests CoBa's compatibility with and enhanced performance through the utilization of larger models. Finally, we analyze the \textbf{runtime efficiency} of CoBa on both the CodeLlama-13B-Python and Phi-1.5-1.3B models, in comparison to other methods. As expected from our theoretical analysis (see Table~\ref{tab:time-complexity}), CoBa requires a significantly shorter runtime than other validation set-based convergence balancing methods like GradNorm$^*$ and FAMO$^*$, and aligns closely with Uniform, the most straightforward MTL approach. This efficiency further positions CoBa as a practical choice for integrating into MTL frameworks for LLMs.




\begin{table}[t]\footnotesize
    \centering
    % \setlength{\tabcolsep}{6pt}
    \caption{Comparison of the time taken per epoch for experiments on the CC Dataset.}
    \vspace{-1ex}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{\pmb{Method}} & \pmb{Phi-1.5-1.3B} & \pmb{CodeLlama-13B-Python} \\
        & \pmb{mins/epoch} & \pmb{mins/epoch} \\
        % \pmb{Method} & \pmb{Phi-1.5-1.3B(mins/epoch)} & \pmb{CodeLlama-13B-Python(mins/epoch)} \\
        \midrule
        Uniform & 22.98 & 188.93 \\
        GradNorm & 25.80 & 197.10 \\
        GradNorm$^{*}$ & 46.08 & 351.13 \\
        LBTW & 26.15 & 195.28 \\
        LBTW$^{*}$ & 29.20 & 234.77 \\
        FAMO & 24.83 & 192.53 \\
        FAMO$^{*}$ & 41.58 & 335.82 \\
        CoBa & 29.05 & 230.20 \\
        \bottomrule
    \end{tabular}}
    \label{tab:5languages-time}
    \vspace{-3ex}
\end{table}

==> contents/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Multi-task learning (MTL) entails simultaneously training of several tasks with the aim of outperforming the benchmarks established by training each task in isolation~\cite{caruana1997multitask,ruder2017overview}. The general idea of the majority of existing works is to encourage positive knowledge transfer throughout the learning process while reducing negative knowledge transfer (dubbed interference) as much as possible~\cite{aribandi2021ext5,liu2024famo}. In the era of advanced Natural Language Processing (NLP), MTL has shown substantial superiority over single-task learning (STL) in both performance and storage efficiency, as corroborated by numerous studies~\cite{liu2017adversarial,jean2019adaptive,aribandi2021ext5,aghajanyan2021muppet}. Nevertheless, MTL faces a critical challenge: task imbalance. Without a properly strategy to equitably balance among tasks, certain tasks may absolutely dominate the training process and hurt the performance of other tasks~\cite{mao2022metaweighting,liu2023mftcoder}.

% In MTL, researchers primarily tend to adopt two methods to mitigate task imbalance: loss balance approaches~\cite{kendall2018multi,chen2018gradnorm,mao2022metaweighting} and gradient manipulation techniques~\cite{desideri2012multiple,sener2018multi,liu2024famo}. The former approach adaptively allocate weights to each task based on heuristic rules to ensure task balance. The latter techniques suggest the formation of novel update vectors for each optimization iteration by linearly combining the gradients of various tasks. While these methodologies have been validated on small-scale models and straightforward classification tasks, their application to state-of-the-art LLMs hindered due to several constraints:
% \begin{itemize}
%     \item Training acceleration techniques such as ZeRO~\cite{rajbhandari2020zero} and FSDP~\cite{zhao2023pytorch} divide model gradients, which renders these methods less compatible with current parallel training frameworks.
%     \item The considerable computational demands of these approaches may slow down training, such as two rounds of forward and backward in per iteration.
%     \item The reduced learning rates prevalent in training LLMs impair the potential efficacy of these strategies.
% \end{itemize}
% Despite work such as Muppet~\cite{aghajanyan2021muppet} and ExT5~\cite{aribandi2021ext5} establishing the feasibility of simple MTL techniques in LLMs, they have not satisfactorily address the problem of task imbalance.

% Furthermore, these studies calculate task weights based on training losses or associated gradients, inadvertently disregarding the critical gap between training and validation losses. A recent work~\cite{mao2022metaweighting} highlights this gap and leverage meta-learning concepts to effectively narrow this gap, thereby enhancing the model's generalization capabilities. This gap is further evidenced by the heterogeneous convergence speeds among tasks. Specifically, the validation loss of certain tasks may continue to converge while others have begun to diverge. Balance in convergence is beneficial to ensure that each task simultaneously approaches the lowest point of its validation loss, avoiding the situation of overfitting on the validation set for certain tasks, and thus substantively boosting overall performance. The aforementioned studies have not successfully attained an balance in task convergence. It is imperative that this issue be addressed to further refine the efficacy of MTL frameworks. 

% To this end, this paper introduces a novel approach that leverages convergence ratios on validation set to dynamically adjust the weight of training loss per task. Thus this method facilitates the economical training of LLMs and achieves convergence balance. 

%In recent years, large language models (LLMs) have emerged as a focal point of research within both the academia and industry, owing to their superior performance. However, the computation and storage demands of training such models are considerably high, rendering the approach of allocating a distinct large model for each task environmentally and resource-wise unsustainable.

In recent years, large language models (LLMs) have emerged as a focal point of research within both the academia and industry, owing to their superior performance. These models are initially subjected to a pretraining stage, designed to ensure they possess broad applicability across a variety of downstream tasks. This is followed by a finetuning stage, which meticulously adapts the models for specific tasks or scenarios. However, this phase requires individual, task-specific finetuning, leading to a complex deployment scenario in production environments. The need to deploy separate models for each specific task, combined with their considerable size and the associated resource consumption, presents a formidable challenge as and number of tasks grows.

%Multi-task learning (MTL) emerges as an effective solution to this dilemma, enabling the joint training of several tasks simultaneously with the aim of outperforming the benchmarks established by training each task in isolation~\cite{caruana1997multitask,ruder2017overview}. This approach not only substantially conserves resources but also facilitates the mutual enhancement of performance across related tasks, even to generalize to entirely unseen tasks. Furthermore, the vast parameter space inherent in large models allows for a comprehensive fitting to multiple tasks, a capability convincingly demonstrated by ChatGPT, which is powered by both GPT-3.5 and GPT-4 OpenAI~\cite{achiam2023gpt}. This underscores the necessity for research into efficient, scalable, and sustainable MTL methodologies that leverage the intrinsic capabilities of large models while addressing their resource-intensive nature.

Multi-task learning (MTL) presents a promising remedy to the above issue by enabling the simultaneous training of multiple tasks~\cite{crawshaw2020multi,vandenhende2021multi,zhang2023survey}. This approach leverages a single model to support a variety of tasks, thus significantly conserving resources. Moreover, MTL not only fosters performance improvements across related tasks but also has the potential to generalize to unseen tasks. On the other hand, the vast parameter space of LLMs facilitates this adaptability, allowing them to undertake multiple tasks simultaneously. This proficiency is exemplified by GPT-3.5 and GPT-4 from OpenAI~\cite{achiam2023gpt}.


\begin{comment}
To efficiently implement multi-task learning on large language models, it is essential to satisfy the following requirements:
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item Low time complexity to ensure that the model can be trained efficiently.
    \item The ability to address the issue of task imbalance in MTL, such as data balance and convergence balance.
\end{itemize}
\end{comment}

For an effective implementation of MTL in LLMs, two critical criteria must be met concurrently. First, \textbf{the approach should incur minimal extra computational costs} since the training of LLMs in itself is already highly resource-intensive. Second, \textbf{it is imperative to guarantee the simultaneous convergence of all tasks}, tactfully navigating to a shared optimal checkpoint.


\begin{table}[t]
    \centering
    % \setlength{\tabcolsep}{6pt}
    \caption{The time complexity of existing MTL approaches for each heterogeneous batch. '$F$' and '$B$' denots the time complexity of the forward and backward propagation respectively, '$K$' is the number of tasks, $\lvert\theta_{s}\rvert$ is the weights (usually the final layer of weights which are shared between tasks), '$a_{i}$' refers to irrelevant constants, '$N$' is the length of history window, '$T$' is to number of training iterations, and $^*$ means the loss weight is determined by the convergence trend of the validation rather than the training loss.}
    \vspace{-1ex}
    % \resizebox{\linewidth}{!}{
    % \begin{tabular}{lc}
    %     \toprule
    %     \pmb{Method} & \pmb{Time Complexity} \\
    %     \midrule
    %     Uniform & $\gO(a_{1}F+a_{2}B)$ \\
    %     GradNorm & $\gO(a_{1}F+a_{2}B+K\lvert\theta_{s}\rvert)$ \\
    %     GradNorm$^{*}$ & $\gO(2(a_{1}F+a_{2}B)+K\lvert\theta_{s}\rvert)$ \\
    %     LBTW & $\gO(a_{1}F+a_{2}B + K)$ \\
    %     LBTW$^{*}$ & $\gO(a_{3}F+a_{2}B + K)$ \\
    %     FAMO & $\gO(a_{1}F+a_{2}B+a_{4}K+a_{5}K^{2})$ \\
    %     FAMO$^{*}$ & $\gO(2(a_{1}F+a_{2}B)+a_{4}K)$ \\
    %     MetaWeighting &  $\gO(K(a_{1}F+a_{2}B))$ \\
    %     CoBa & $\gO(a_{3}F+a_{2}B+a_{6}K)$ \\
    %     \bottomrule
    % \end{tabular}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \pmb{Method} & & & & & & \pmb{Time Complexity} \\
        \midrule
        Uniform & & & & & & $\gO(a_{1}F+a_{2}B)$ \\
        GradNorm & & & & & & $\gO(a_{1}F+a_{2}B+K\lvert\theta_{s}\rvert)$ \\
        GradNorm$^{*}$ & & & & & & $\gO(2(a_{1}F+a_{2}B)+K\lvert\theta_{s}\rvert)$ \\
        LBTW & & & & & & $\gO(a_{1}F+a_{2}B + K)$ \\
        LBTW$^{*}$ & & & & & & $\gO(a_{3}F+a_{2}B + K)$ \\
        FAMO & & & & & & $\gO(a_{1}F+a_{2}B+a_{4}K+a_{5}K^{2})$ \\
        FAMO$^{*}$ & & & & & & $\gO(2(a_{1}F+a_{2}B)+a_{4}K)$ \\
        MetaWeighting & & & & & &  $\gO(K(a_{1}F+a_{2}B))$ \\
        CoBa & & & & & & $\gO(a_{3}F+a_{2}B+a_{6}K)$ \\
        \bottomrule
    \end{tabular}}
    \label{tab:time-complexity}
    \vspace{-3ex}
\end{table}
%This metric reflects the number of forward and backward propagation rounds required per training iteration.
%Traditional methodologies in MTL, notably those based on loss balance~\cite{kendall2018multi,chen2018gradnorm,mao2022metaweighting} and gradient manipulation~\cite{desideri2012multiple,sener2018multi,liu2024famo}, have established their efficacy within the small scale models and straightforward classification tasks. Notwithstanding, the translation of these established approaches to LLMs is met with considerable resistance. Illustratively, the table~\ref{tab:computational-complexity} highlights that techniques such as FAMO~\cite{liu2024famo} and MetaWeighting~\cite{mao2022metaweighting} mandate at least two complete forward and backward propagation rounds within a heterogeneous training batch (a blend of data samples from diverse tasks). Further contributing factors will be discussed in detail in the Section~\ref{sec:related_work}.

%On the other hand, works such as Muppet and ExT5 have validated the practicality of straightforward MTL approaches in LLMs, concurrently incorporating the more challenging generative tasks. Yet, these approaches have not made attempts to solve the prevalent challenge of task convergence imbalance within MTL environments. This leads to a phenomenon where certain tasks may still be converging, while others begin to diverge, potentially deteriorating the overall performance of the model. 

Unfortunately, current approaches do not simultaneously meet the above two requirements. Traditional MTL methods, particularly those focusing on loss balancing and gradient manipulation~\cite{kendall2018multi,chen2018gradnorm,mao2022metaweighting,liu2024famo}, have proven effective for smaller models and straightforward classification tasks. However, adapting these established techniques to LLMs presents significant challenges due to the high computational costs and the complexities involved in integrating them with parallel training frameworks. For example, GradNorm~\cite{chen2018gradnorm}, FAMO~\cite{liu2024famo}, and MetaWeighting~\cite{mao2022metaweighting} typically incurs a high computational cost with regard to the number of tasks $K$, as shown in Table~\ref{tab:time-complexity}. Conversely, NLP models such as Muppet~\cite{aghajanyan2021muppet} and ExT5~\cite{aribandi2021ext5} employ a straightforward data mixing strategy from multiple tasks for application in LLMs. However, they fall short of addressing the persistent issue of uneven task convergence within MTL settings. This imbalance can result in a scenario where some tasks are still optimizing while others begin to worsen, negatively impacting the model's overall effectiveness.


%To conduct uncomplicated, low-consumption multi-task training on LLMs and to achieve convergence balance across tasks, this paper introduces an innovative MTL methodology. 
In this paper, we introduce \textbf{CoBa} (COnvergence BAlancer), an innovative MTL approach designed for LLMs. This method aims to achieve balanced convergence across various tasks while maintaining ease of applicability in the training of LLMs. The core strategy involves dynamically varying each task's training loss weight based on its convergence trends in the validation dataset. Two essential criteria underpin this method are: 1) \textbf{when the validation losses of all tasks consistently decline, the method lowers weights for those converging faster (experiencing steeper drops in validation losses) and increases weights for those converging more gradually (exhibiting less steep slopes).} 2) \textbf{For any tasks showing divergence—a signal of possible overfitting—their associated weights are decreased. On the other hand, weights are boosted for tasks that are steadily converging.} To move forward to these objectives, we introduce the Relative Convergence Score (RCS) to address the first criterion and the Absolute Convergence Score (ACS) for the second. A Divergence Factor (DF) is then applied to ascertain which score prevails in influencing the final weight allocation. Note that RCS, ACS, and DF are all efficiently computed, leveraging the validation loss slopes through normalization and softmax functions, making them not only computationally effective but also easily compatible with parallel training architectures. To summarize, the main contributions of our study are: %Empirical results from experiments conducted on three real-world datasets demonstrate that our proposed "CoBa" method effectively maintains balance in convergence across varied experimental settings.} Moreover, it yields a notable performance enhancement, with up to a $5\%$ relative improvement in the majority of the scenarios tested.

\begin{comment}
    This approach dynamically adjust the weight of training loss per task via monitoring convergence ratios on validation set. 
Specifically, by modeling the slope of each task's validation loss across a previous interval of training iterations, our method captures the convergence slope for each task during that period. Thereafter, the allocation of per task training loss weight follows two fundamental principles: 
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item Tasks exhibiting more rapid convergence are assigned lesser weights, while those with slower convergence receive greater weights.
    \item Tasks nearing divergence on validation loss are given lesser weights, in contrast to tasks that manifest ongoing convergence, which are assigned greater weights.
\end{itemize}
In this way, our method effectively achieves convergence balance across multiple tasks with little overhead-requiring only one additional forward pass per iteration. 

In order to verify the effectiveness of the method proposed in this paper, we conduct a series of experiments using three distinct multi-task datasets. These datasets encompass a code completion dataset spanning five different programming languages, a collection of datasets comprising five distinct code-related tasks, and the QA in language dataset derived from XTREME-UP~\cite{ruder2023xtreme}. The results of experiments demonstrate that our method facilitates convergence balance across all three experimental settings, and delivers a relative improvement of up to 5\% in most scenarios.
\end{comment}


\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item We introduce the CoBa, a novel strategy designed to achieve a state of balanced convergence across various tasks. This approach is straightforward in its application to LLMs, bridging the gap between advanced multitask learning requirements and practical usability.
    \item We propose two new metrics — the RCS and the ACS — along with a DF. The former two cater to the aforementioned two criteria respectively, while the DF determines which metric primarily affects the final weight distribution.
    \item We validate the efficacy and efficiency of CoBa through extensive experiments and show that CoBa not only maintains balanced convergence across tasks but also achieves up to a 13\% relative performance improvement in comparison with the second-best baselines.
\end{itemize}

%RCS is utilized to decrease weights for tasks showing rapid convergence and to increase weights for those converging more slowly, whereas ACS targets the reduction of weights for tasks demonstrating signs of divergence.

%We intduce a computationally simple yet effective MTL method for LLMs that achieves convergence balance across multiple tasks.
% These resources will be made publicly available to facilitate further advancements within the field.
%We conduct extensive experiments across three multi-task datasets, demonstrating that our proposed method achieves convergence balance and results in a relative improvement of up to 5\% in most cases.
    %\item We meticulously curate two multi-task datasets that will be invaluable assets to the research community. They include a code completion dataset spanning five programming languages and another dataset that addresses five distinct code-related tasks. 



==> contents/limitations.tex <==
\section{Ethical Considerations}
Our research is foundational and is not expected to have significant social implications. We ensure transparency and adherence to ethical standards in the use of datasets. Additionally, the accessibility of these datasets is beneficial for broader reproducibility and review within the research community, aligning with ethical research practices. However, we acknowledge the responsibility that comes with the development of any multi-task learning technology. We encourage ongoing dialogue and ethical considerations in the application of our research findings.

\section{Limitations}
We have identified the main limitations of our approach as follows:
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item \textbf{The Model Parameter Scale:} Due to resource constraints, we are unable to evaluate the efficacy of CoBa on larger LLMs. In future work, we aspire to conduct experiments with larger LLMs, akin to MFTCoder~\cite{liu2023mftcoder}, to further substantiate our findings.
    \item \textbf{The Number of Tasks:} Due to the limited number of open-source multi-task fine-tuning data, we are unable to experiment on more tasks. In the future, we hope to collect more relevant multi-task datasets to verify the effectiveness of CoBa.
    \item \textbf{Domain of application:} This paper focuses on NLP. However, multi-task learning is not limited to this modality. In the future, we aim to explore other modalities such as computer vision.
\end{itemize}

==> contents/method.tex <==
\section{CoBa Method}
\label{sec:method}


Multi-task learning (MTL) is engineered to optimize a single model, parameterized by ${\theta} \in {\sR^m}$, enabling it to adeptly perform $K \geq 2$ tasks, potentially even in tandem. The loss function for task $i$ at the $t$-th iteration is denoted by ${\ell_i(\theta;t)}:{\sR^m}\rightarrow{\sR_{\geq 0}}$. This forms the foundation for the optimization challenge of MTL, expressed as:
\begin{equation}
    \mathop{\min}_{\theta \in \sR^m} \left\{\ell(\theta;t) := \mathop{\sum}_{i=1}^{K}{\omega_{i}(t) \ell_i(\theta;t)} \right\},
\label{eqa:1}
\end{equation}
where $\omega_{i}(t)$ is the loss weight for task $i$ at iteration $t$. Assigning $\omega_{i}(t) = 1/K$ ensures data balance, giving due attention to tasks irrespective of their sample sizes. However, this approach leads to varying convergence rates across tasks (e.g., see Figure~\ref{fig1-a}), complicating the identification of a checkpoint that is optimal for all tasks. Our goal is to adjust the weights $\omega_{i}(t)$ to harmonize these convergence rates. Furthermore, We prioritize generalization over mere training performance, and so the weights $\omega_{i}(t)$ is derived from the validation rather than training losses. To achieve these objectives, we adhere to two key criteria:

\textbf{\textit{c1}}.~ When validation losses for all tasks are on a downward trend, tasks with faster convergence (sharper decline) receive reduced weights to avoid rapid overfitting. In contrast, tasks converging more slowly (gentler slopes) are assigned increased weights to encourage more learning.

\textbf{\textit{c2}}.~When any tasks begin to display signs of divergence (overfitting), their weights are decreased. Conversely, tasks that maintain a convergence trajectory are accorded higher weights.

These two criteria are quantified respectively through Relative Convergence Scores (RCS) and Absolute Convergence Scores (ACS). RCS is employed to assess the convergence pace relative among tasks, while ACS measures the current convergence rate against historical rates for each task individually. Note that these scores are derived from the slopes of validation losses—not the gradients—to minimize computational demands. We then integrate a divergence factor (DF), highlighting the overall convergence trajectory across tasks. This factor ensures RCS impacts weights predominantly when all tasks are converging, while ACS takes precedence as any commence diverging. In the sequel, we detail the computation of slopes, the formulation of RCS and ACS, and their amalgamation with the DF.




%This section details the proposed MTL method, which is designed to address the issue of imbalance convergence across tasks. Firstly, we randomly sample a mini validation batch in each training iteration to calculate the loss ratio. And we fit a linear polynomial $\alpha x + \beta$ to obtain the convergence slope for each task. Then we calculate relative convergence scores and absolute convergence scores. Finally, we combine the relative and absolute scores to assign a weight to the training loss of each task.

\begin{figure*}[t]
    \centering
    \subfigure{
    \includegraphics[width=0.4\linewidth,origin=c]{images/3tasks_legend.pdf}}\\
    \vspace{-2.5ex}
    \clearsubcaptcounter
    \subfigure[\scriptsize Loss ratios.]{
        \includegraphics[height=0.134\linewidth]{images/3tasks_loss_ratio.pdf}
        \label{fig1-a}
    }
    \hspace{-2ex}
    \subfigure[\scriptsize Convergence slopes.]{
        \includegraphics[height=0.13\linewidth]{images/3tasks_slope.pdf}
        \label{fig1-b}
    }
    \hspace{-2ex}
    \subfigure[\scriptsize Relative scores.]{
        \includegraphics[height=0.13\linewidth]{images/3tasks_relative_score.pdf}
        \label{fig1-c}
    }
    \hspace{-2ex}
    \subfigure[\scriptsize Absolute scores.]{
        \includegraphics[height=0.13\linewidth]{images/3tasks_absolute_score.pdf}
        \label{fig1-d}
    }
    \hspace{-2ex}
    \subfigure[\scriptsize Divergence factor.]{
        \includegraphics[height=0.133\linewidth]{images/3tasks_divergence_factor.pdf}
        \label{fig1-e}
    }
    \hspace{-2ex}
    \subfigure[\scriptsize Weights.]{
        \includegraphics[height=0.13\linewidth]{images/3tasks_weight.pdf}
        \label{fig1-f}
    }
    \vspace{-2ex}
    \caption{Demonstration of CoBa's task weight calculation process based on a real example.}
    \label{fig1}
    \vspace{-3ex}
\end{figure*}

\begin{comment}
\subsection{Multitask Learning (MTL)}
\label{subsec:mtl}
Consider a multi-task learning problem is  optimizing a single model with parameter ${\theta} \in {\sR^m}$ that can perform $k \geq 2$ well, where the loss function of each task at the $t$-th iteration refers to ${\ell_i(\theta;t)}:{\sR^m}\rightarrow{\sR_{\geq 0}}$. Consequently, it is a standard approach to minimize the loss weighted by $\omega_{i}(t)$ across all tasks:
\begin{equation}
    \mathop{\min}_{\theta \in \sR^m} \left\{\ell(\theta;t) := \mathop{\sum}_{i=1}^{k}{\omega_{i}(t) \ell_i(\theta;t)} \right\}.
\label{eqa:1}
\end{equation}

We aim to learn the functions $\omega_{i}(t)$ with the following goals, thus achieving convergence balance:
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item Tasks with more rapid convergence speeds (steeper slopes) are assigned smaller weights, while those with slower convergence speeds (flatter slopes) are allocated larger weights.
    \item Tasks whose validation loss is nearing divergence are assigned smaller weights, while those that continue to converge are allocated larger weights.
\end{itemize}
\end{comment}

\subsection{Convergence Slope}

The convergence speed of different tasks can be intuitively measured by examining the slope of the validation loss curves. Figure~\ref{fig1-a} depicts this scenario, where Task B, marked by the green curve, demonstrates a quicker convergence compared to Task C, which is represented by the red curve, up until step 5900. This is reflected in the steeper slope observed for Task B, indicating a higher absolute value for its convergence slope than that of Task C as shown in Figure~\ref{fig1-b}.

To ensure a fair comparison of convergence speeds across tasks, we first normalize the validation losses. We achieve this normalization by using the validation loss ratio, $\Bar{\ell}_i^{val}(\theta;t)$, calculated as the current validation loss divided by the initial validation loss at step 0, according to the formula:
\begin{equation}
    \Bar{\ell}_i^{val}(\theta;t) = \frac{\ell_i^{val}(\theta;t)}{\ell_i^{val}(\theta;0)},
\label{eqa:2}
\end{equation}
where the $\ell_i^{val}(\theta;0)$ refers to the validation loss of the $i$-th task at step 0. Utilizing this normalized validation loss ratio, $\Bar{\ell}_i^{val}(\theta;t)$, we fit a linear model defined by $\alpha x + \beta$ across a selected range of iterations. The slope $\alpha$ from this linear fit provides us with an estimate of the convergence slope for that period. More specifically, at iteration $t$, we construct the observations vector $\vx_{i}(t) = [t,1]^\top$ and accordingly compile the observation matrix $\mX_{i}(N;t) = [\vx_{i}(s_0),...,\vx_{i}(t)]^\top$, matched with the corresponding validation loss ratios $\vy_{i}(N;t) = [\Bar{\ell}_i^{val}(\theta;s_0),...,\Bar{\ell}_i^{val}(\theta;t)]^\top$, where $\vx^\top$ denotes the transpose of $\vx$, $N$ refers to the length of history window, and $s_0 = \mathop{\max}(0, t-N+1)$. We aim to obtain the coefficient vector $\vc_i(N;t) = [\alpha_{i}(N;t),\beta_{i}(N;t)]^\top$, which minimizes the MSE between the projected values $\mX_{i}(N;t)\vc_{i}(N;t)$ and the actual values $\vy_{i}(N;t)$:
\begin{equation} 
\vc_{i} = \argmin_{\vc_{i}}\frac{1}{2}(\mX_{i}\vc_{i}-\vy_{i})^{\top}(\mX_{i}\vc_{i}-\vy_{i}). 
\label{eqa:6} 
\end{equation}
The vector $\vc_i(N;t)$ has a closed-form solution as:
\begin{equation} 
\vc_{i} = (\mX_{i}\mX_{i}^{\top})^{-1}\mX_{i}\vy_{i}^{\top}. \label{eqa:7} 
\end{equation}
It is critical to note that the solution in Eq.~\eqref{eqa:7} is only applicable for $t \geq 2$. For this reason, we set $\alpha_{i}(N;t)=0$ when $t<2$.

Furthermore, acknowledging the potential inaccuracy of initial convergence slopes as given by Eq.~\eqref{eqa:7}, our methodology introduces a parameter $W$ analogous to warm-up steps: starting from step $W$, the process for updating the weights $\omega_i(t)$ attributed to the training loss to being determined by the convergence slopes observed within a specific sliding window period. Prior to reaching this step, however, the weights allocated to all tasks are uniformly set at $1/K$, ensuring a balanced starting point. The configuration of both $N$ and $W$ is linked to the total number of batches within the validation set. Given that the validation set is partitioned into $M$ batches, with each iteration utilizing only a single mini-batch from the validation set for calculating the task-specific loss weight $w_i(t)$, we recommend setting $N$ at $2M$ and $W$ at $M$.

\begin{comment}
\subsection{Loss Ratio}
Due to the varying scales of loss across different tasks, tasks with larger loss scales could dominate the assessment of the overall validation loss, which is not conducive to a fair evaluation of the multi-task performance. Hence, we draw inspiration from the GradNorm approach and utilize the overall validation loss ratio to measure the state of convergence in multitask learning. For each task, the validation loss ratio is used in place of the raw validation loss:
\begin{equation}
    \Bar{\ell}_i^{val}(\theta;t) = \ell_i^{val}(\theta;t) / \ell_i^{val}(\theta;0),
\label{eqa:2}
\end{equation}
where the $\ell_i^{val}(\theta;0)$ refers to the validation loss of the $i$-th task at step 0. $\Bar{\ell}_i^{val}(\theta;t)$ represents the inverse training rate metric for task $i$ (i.e., a lower $\Bar{\ell}_i^{val}(\theta;t)$ value corresponds to a faster training rate for task $i$).

\subsection{Convergence Slope}
Intuitively, the slope of a loss curve denotes the rate at which the curve converges. In order to forecast the convergence rate of the validation loss curve for a specific task, this study employs the ratio of validation losses across a continuous interval of training iterations to fit a polynomial curve of the form $\alpha x + \beta$. The coefficient $\alpha$ is interpreted as the slope of this interval of the curve, namely convergence slope.

Assume that the training has advanced to the $t$-th iteration, the sequence of validation loss rates for task $i$ is characterized by:
\begin{equation}
    Y_{i}(N;t) = [y_{i}(start),...,y_{i}(t)]^\top,
\label{eqa:3}
\end{equation}
where $y_{i}(t) = \Bar{\ell}_i^{val}(\theta;t)$, $N$ refers to the length of history window, and $start = \mathop{\max}(0, t-N+1)$. And we formulate the observations at $t$-th step as $x_{i}(t) = [t,1]^\top$, thus the sequence of observation in this training interval is given by:
\begin{equation}
    X_{i}(N;t) = [x_{i}(start),...,x_{i}(t)]^\top.
\label{eqa:4}
\end{equation}

We introduce a coefficient matrix as $W_i(N;t) = [\alpha_{i}(N;t),\beta_{i}(N;t)]^\top$, and fit the straight line through the following formula:
\begin{equation}
    Y_{i}(N;t) = X_{i}(N;t)W_{i}(N;t).
\label{eqa:5}
\end{equation}

The optimization objective when fitting the aforementioned linear polynomial is to minimize the distance between $X_{i}W_{i}$ and $Y_{i}$:
\begin{equation}
    W_{i} = \mathop{\arg\min}_{W_{i}}\frac{1}{2}(X_{i}W_{i}-Y_{i})^{\top}(W_{i}X_{i}-Y_{i}).
\label{eqa:6}
\end{equation}

Subsequently, the matrix $W_{i}$ can be derived using the closed form:
\begin{equation}
    W_{i} = (X_{i}X_{i}^{\top})^{-1}X_{i}Y_{i}^{\top}.
\label{eqa:7}
\end{equation}

In conclusion, we define the per task convergence slope and the total convergence slope as:
\begin{equation}
    s_{i}(t) = 
    \left\{
    \begin{array}{lr}
        0, & t \le 2, \\
        \alpha_{i}(N;t), & t > 2.
    \end{array}
    \right.
\label{eqa:8}
\end{equation}
% \begin{equation}
%     s(t) = \frac{1}{k} \mathop{\sum}_{i=1}^{k} s_{i}(t).
% \label{eqa:9}
% \end{equation}

To intuitively demonstrate the dynamics of the convergence slope, we plot figures that depict the relationship between convergence slope and validation loss ratios through graphical curves corresponding to three distinct tasks, as illustrated in Figure \ref{fig1-a} and \ref{fig1-b}. It is explicitly indicate that an increase in the convergence slope is concomitant with the convergence of the loss ratio.

% In conclusion, the total convergence slope is computed as:
% \begin{equation}
%     s(t) = \frac{1}{N} \mathop{\sum}_{i=1}^{k} s_{i}(t)
% \end{equation}
\end{comment}



%\subsection{Balancing Convergence with Convergence Slopes}
%Prior to each computation of training loss, we randomly sample a mini-batch from the validation set and calculate the ratio of validation loss for each task. For every task, a sliding window of length $N$ is maintained to record the validation loss ratios for the previous $N$ steps, denoted by $\gL_{i}(t)=[\ell_{i}(\theta;t-N+1),...,\ell_{i}(\theta;t)]$. Leveraging the $\gL_{i}(t)$, we proceed to infer the convergence slope $s_{i}(t)$ for each task. In parallel, we also preserve a sliding window sequence of convergence slope of length $N$ for convenient reference in later stages, which can be formulated as $\gS_{i}(t) = [s_{i}(t-N+1),...,s_{i}(t)]$.

%Furthermore, our method introduces a parameter that resembles warm-up steps, referred to as $\gW$. This parameter dictates that commencing from step $\gW$, the update mechanism for the weights assigned to the training loss will be governed by the convergence slopes recorded within the sliding window. The setting of parameter $N$ and $\gW$ is associated with the number of batches in the validation set. Assuming that the validation set is divided into $m$ batches after batch processing, it is advisable to set $N$ to $10m$ and $\gW$ to $m$. Before this step, the weights for all tasks are equal.


\subsection{Relative Convergence Scores (RCS)}
As mentioned above, the goal of RCS is to dynamically allocate smaller weights to tasks that are converging more rapidly, and larger weights to those converging more slowly, such that all tasks can converge at the same time. This score is calculated based on the convergence slopes of all tasks at a specific iteration $t$, that is,
\begin{equation} 
\RCS_i(t) = \softmax_i\bigg(\frac{K \alpha_{i}(t)}{\sum_{i=1}^{K} \lvert \alpha_{i}(t) \rvert}\bigg), \label{eqa:RCS} 
\end{equation} 
where $\softmax_i$ means that the softmax operation is applied to the dimension of $i$ (i.e., the dimension of tasks). To guarantee a level playing field across all tasks, we first normalize the convergence slopes as $\alpha_{i}(t) / \sum_{i=1}^K |\alpha_{i}(t)|$, making the calculated score resistant to variations in the mean scale of the slopes. However, given that this normalized value tends towards zero as the number of tasks $K$ increases, we compensate by the multiplication of $K$. This adjustment ensures that the final RCSs are not disproportionately affected by the total number of tasks being considered. The subsequent application of the softmax function can then effectively differentiate the RCS values across the tasks.

In practice, as displayed in Figure~\ref{fig1-a}, Task B, highlighted by the blue curve, demonstrates the slowest convergence rate, which is appropriately reflected by the highest RCS, depicted in Figure~\ref{fig1-c}. Additionally, Figure~\ref{fig1-a} shows that Task C (the red curve) converges slower than Task A (the green curve) up to step 8000, which is coherently translated into a higher RCS for Task C compared to Task A when $t \leq 8000$ (cf. Figure~\ref{fig1-c}).


\begin{comment}
\subsubsection{Relative Convergence Scores}
In pursuit of the first objective mentioned in Section~\ref{subsec:mtl}, we try to quantify the relative convergence speeds with relative convergence scores computed by the convergence slopes. We normalize the convergence slopes for all tasks at step $t$:
\begin{equation}
    RN_{i}(t) = \frac{k \times s_{i}(t)}{\mathop{\sum}_{i=1}^{k} \lvert s_{i}(t) \rvert}. 
\label{eqa:9}
\end{equation}
Then we feed $RN(t) = (RN_{1}(t),...,RN_{k}(t))$ into a $\softmax$ function to obtain the relative convergence scores among tasks:
\begin{equation}
    \begin{array}{lr}
        score^{rel}(t) = \softmax (RN(t)).
    \end{array}
\label{eqa:10}
\end{equation}
Equation \ref{eqa:9} preserves the innate sign attributes of the individual slopes, and maps them onto an interval that is more responsive to the $\softmax$ function. This mapping facilitates to produce a properly disparity in the resultant scores following the $\softmax$ function. As a result, Equation \ref{eqa:10} assigns lower weights to tasks with lower convergence slope values (steeper slopes), owing to their rapid convergence speeds. In contrast, tasks with higher convergence slope values (flatter slopes) are afforded proportionally greater weights, in accordance with their slow convergence speeds.

Figure \ref{fig1-a}, \ref{fig1-b} offers a visual illustration of the trends for relative convergence scores:
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item Task B exhibits the most rapid convergence speed with respect to loss ratio, as evidenced by the correspondingly greatest convergence slope values. Consequently, it garners the highest proportion of relative convergence scores.
    \item Before 8000 steps, Task C demonstrates a swifter loss ratio convergence when compared to Task A, maintaining a predominantly larger convergence slope values during this interval. This results in a greater allocation of relative convergence scores to Task A over Task C. After 8000 steps, this trend undergoes a reversal.
\end{itemize}
\end{comment}




\subsection{Absolute Convergence Scores (ACS)}
Unfortunately, relying solely on RCS proves to be inadequate for the needs of multi-task learning. As depicted in Figures~\ref{fig1-a} and~\ref{fig1-c}, Task B illustrates a scenario where, despite beginning to diverge, it still secures the highest RCS due to its largest (albeit positive) convergence slope. Awarding the greatest weight to Task B under these circumstances could exacerbate the situation by leading to further overfitting on this task, potentially causing overall model performance to deteriorate—a scenario we intend to avoid. This predicament underscores the necessity of ACS, whose fundamental purpose is to mitigate such risks by allocating reduced weights to tasks that are diverging, while favoring tasks that are on a converging trajectory with larger weights. The ACS for a given task $i$ at any step $t$ is mathematically represented as:
\begin{equation}
\ACS_i(t) = \softmax_i\bigg(\frac{-N\alpha_i(t)}{\sum_{j=t-N+1}^t \lvert \alpha_i(j) \rvert}\bigg).
\label{eqa:ACS}
\end{equation}
Unlike RCS, where both normalization within the softmax and the softmax itself occur across the task dimension $i$, ACS performs normalization along the iteration dimension $t$ from step $t-N+1$ to step $t$, but subsequently applies the softmax function across the task dimension $i$. ACS's unique aspect lies in its exclusive consideration of a task's own historical performance during the normalization, without considering other tasks. This isolation of individual task trajectory is the reason behind the nomenclature ``Absolute'' in ACS.


In general, in the initial stages of fine-tuning, tasks typically exhibit fast convergence, marked by a substantial negative slope. For tasks that maintain a consistent convergence, these negative slopes exhibit minimal change over the span from $t-N+1$ to $t$. In contrast, tasks that start to diverge will show significant changes in their slopes, transitioning from negative to neutral or even positive values. By normalizing the slope over this time window and accounting for the negative sign as shown in Eq.~\eqref{eqa:ACS}, tasks that continue to converge receive relatively high values at step $t$. Conversely, tasks that begin to diverge are assigned progressively lower values. The subsequent application of the softmax function across tasks allows us to allocate weights appropriately, thereby achieving the desired effect of bolstering converging tasks and restraining the influence of diverging ones.


Figure \ref{fig1-a}, \ref{fig1-b} and \ref{fig1-d} intuitively demonstrates the utility of the ACSs. Since Task B's loss ratio diverges earliest, its convergence slope is the quickest to approach zero. Once this trend of fastest divergence is captured, Task B will receive the smallest ACS. Addtionally, before step 5900, Task C's convergence slope value approaches zero faster than Task A's, thereby receiving a lower ACS. After 5900 steps, the convergence slope value of Task A exceeds Task C's, indicating that Task A will diverge earlier than Task C, thus a lower ACS is attributed to Task A.



%However, only having relative convergence scores is insufficient because when Task B begins to diverge, it still has the largest convergence slope value, resulting in the highest relative convergence score. Such dominance by a diverging task during the training phase can induce global divergence and ultimately degrade model performance, which is not our desired outcome.

%In an effort to materialize the second objective outlined in Section~\ref{subsec:mtl}, our method introduces absolute convergence score to quantify the absolute convergence speed for each task independently. 

\begin{comment}
Firstly, we concatenate the convergence slope $\gS_{i}(t)$ of all tasks into a matrix of dimensions $k \times N$, denoted by $\widehat{\gS}(t) = \mathop{concat}({\gS}_{1}(t),...,{\gS}_{k}(t))$. Each element in this matrix is represented as:
\begin{equation}
    \widehat{\gS}_{ij}(t) = S_{i}(j).
\label{eqa:11}
\end{equation}
where $i \in [1,k], j \in [t-N+1,t]$. Then we conduct reverse normalization on this matrix:
\begin{equation}
    AN_{ij}(t) = - \frac{(k \times N) \times \widehat{S}_{ij}(t)}{\mathop{\sum}_{i=1}^{k} \mathop{\sum}_{j=t-N+1}^{t} \widehat{S}_{ij}(t)},
\label{eqa:12}
\end{equation}
where $k \times N$ is a scaling factor that amplifies the scale of the normalized scores to an appropriate range. And the negative sign is deliberately employed to exploit the directional property of the convergence slope: a positive value signifies divergence, whereas a negative value denotes convergence. Accordingly, negative values that are proximal to zero denote an trend toward divergence. Subsequent to the first normalization process, tasks with convergence rate values that either approximate zero or surpass it are allocated lesser scores. Then we map these values to a positive range using the $\softmax$ function:
\begin{equation}
    \overline{AN}(t) = \mathop{\softmax}(AN(t)).
\label{eqa:13}
\end{equation}
Finally, we extract the scores corresponding to each task at the $t$-th step from the matrix $\overline{AN}(t)$, subsequently subjecting them to an additional normalization procedure, and obtain the absolute convergence scores for each task:
\begin{equation}
    \widetilde{AN}_{i}(t) = \frac{\overline{AN}_{it}(t)}{\mathop{\sum}_{i=1}^{k} \overline{AN}_{it}(t)}.
\label{eqa:14}
\end{equation}
\begin{equation}
    score^{abs}(t) = (\widetilde{AN}_{1}(t),...,\widetilde{AN}_{k}(t)).
\label{eqa:15}
\end{equation}
% This culminates in the derivation of the absolute convergence scores for each individual task, effectively quantifying their respective convergence statuses within the training regimen.

% reflecting their comparative instability or propensity for divergence within the training landscape.

Notably, we do not adopt the approach of calculating Equations~\ref{eqa:12} and~\ref{eqa:13} individually for each task's $\gS_{i}(t)$ to compute the absolute convergence scores. Because, this method is inadequate for capturing the divergence trend of a task, where its convergence slope oscillates around zero. Consequently, tasks with slow convergence speeds that are nearing divergence would be assigned higher absolute scores, while tasks with fast convergence speeds that are still converging would receive lower absolute scores. Instead, by concatenating the $\gS_{i}(t)$ values of all tasks and computing the absolute convergence scores collectively, we ensure that any task whose convergence slope starts to oscillate near zero is assigned a very small absolute convergence score. Thus, the divergence of certain tasks are effectively suppressed.

Figure \ref{fig1-a}, \ref{fig1-b} and \ref{fig1-d} intuitively demonstrates the utility of absolute convergence scores:
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item Since Task B's loss ratio diverges earliest, its convergence slope is the quickest to approach zero. Once this trend of fastest divergence is captured, Task B will receive the smallest absolute convergence score.
    \item Before step 5900, Task C's convergence slope value approaches zero faster than Task A's, thereby receiving a lower absolute convergence score. After 5900 steps, the convergence slope value of Task A exceeds Task C's, indicating that Task A will diverge earlier than Task C, thus a lower absolute convergence score is attributed to Task A.
\end{itemize}
\end{comment}

\subsection{Divergence Factor and Final Weight}
In practice, it's common that at the onset of training, tasks generally show converging patterns. Consequently, during this phase, RCS should play the primary role in dictating the weights assigned to each task's loss. Nevertheless, as training progresses, it may happen that some tasks begin to diverge. In such instances, ACS ought to take precedence in influencing the task loss weights. To seamlessly transition from RCS-dominance to ACS-dominance in response to these evolving conditions, we introduce the concept of a divergence factor (DF), designed to monitor divergence trends throughout the training process. Given the divergence factor $\DF(t)$ at step $t$, we can compute the final weight vector $\vomega(t) = [\omega_1(t),\cdots,\omega_K(t)]^\top$ that takes both RCS and ACS into account as:
\begin{equation}
\vomega(t) = \DF(t) \RCS(t) + (1-\DF(t)) \ACS(t).
\label{eqa:19}
\end{equation}
Now let us delve into the calculation of $\DF(t)$. The approach to determining the DF involves capturing the largest (considering signs) convergence slope, denoted as $\alpha_{\max}(t)$, across all tasks at each iteration $t$ within the sliding history window. The DF itself is then quantified by the formula:
\begin{equation}
\DF(t) = \min\bigg(t\, \softmax_t\Big(- \frac{\tau t\alpha_{\max} (t)}{\sum_{i=1}^t  \alpha_{\max} (i)} \Big), 1\bigg),
\label{eqa:16}
\end{equation}
where $\softmax_t$ denotes that the softmax operation is applied to the dimension of steps. Crucially, within the softmax function, we multiply the numerator by the current step $t$ to ensure that $\DF(t)$ does not inherently decline as $t$ increases—even though the denominator naturally accumulates over time. The use of the temperature parameter $\tau > 1$ assures a sufficiently high level of distinction between the softmax outputs. Finally, the entire $\softmax$ term is scaled by $t$ to guarantee that $\DF(t)$ equals 1 when all tasks are continuously converging. Concretely, suppose that the most slowly converging task sustains a constant negative slope. The $\softmax$ operation yields $1/t$ at step $t$, suggesting a decreasing proportion of RCS in the final weight as training proceeds. However, in this context where all tasks are converging, RCS should retain its dominance in the final weight. Thus, by multiplying the $\softmax_t$ outputs by $t$, we ensure $\DF(t)$ remains at 1. On the other hand, $\DF(t)$ given by Eq.~\eqref{eqa:16} falls below 1 only when the slope of a task keeps increasing from negative to zero or even positive—indicative of the onset of divergence, which aligns with the intended design of our method.



Illustrating the proposed method with the example provided in Figure~\ref{fig1}, we note that in the initial training stages—say, before 700 steps—the gradual tapering of the DF (see Figure~\ref{fig1-e}) allows RCS to exert a stronger influence, leading to Task B receiving the heaviest weight. However, as Task B's convergence slope swiftly nears zero, the DF undergoes a swift decline, hence amplifying the role of ACS. Our methodology adeptly captures the point at which the convergence slope of Task B starts oscillating around zero, resulting in a lower ACS for Task B. Post the 700-step mark, Task B's weight is reduced significantly, a strategic move to effectively mitigate the risk of overfitting.


\begin{comment}
\subsubsection{Put Everything Together}
Intuitively, relative convergence scores should exert minimal influence on weight adjustments in the presence of task divergence. To better integrate relative scores and absolute scores, we introduce a divergence factor to capture the trend of divergence and to immediately reduce the impact of relative convergence scores. We first record the largest convergence slope $\widetilde{s}(t)$ from all task at each previous step to obtain a sequence $\widetilde{\gS}(t)=[\widetilde{s}(1),...,\widetilde{s}(t)]$. Then we apply inverse normalization to this sequence:
\begin{equation}
    DN_{i}(t) = - \frac{t \times \widetilde{s}(t)}{\mathop{\sum}_{i=1}^{t}\widetilde{s}(t)}.
    \label{eqa:16}
\end{equation}
Following the application of the $\softmax$ function with temperature $k$, we extract the element corresponding to the last position. This element is subsequently multiplied by the current step number to prevent it from decaying too quickly as training steps increases:
\begin{equation}
    D(t) = \softmax(k * DN(t)).
    \label{eqa:17}
\end{equation}
\begin{equation}
    d(t) = D_{t}(t) * t.
    \label{eqa:18}
\end{equation}
where the number of tasks $k$ serves the role of the temperature in the $\softmax$ function. The total score to each task can be expressed as follows:
\begin{equation}
    \begin{split}
        score(t) = d(t) \cdot score^{rel}(t) + \\ (1 - d(t)) \cdot score^{abs}(t).
    \end{split}
\label{eqa:19}
\end{equation}

In conclusion, the weight attributed to each task at $t$-th step can be formulated as:

\begin{equation}
    \begin{split}
        \omega(t) = \mathop{\softmax}(k * score(t)).
    \end{split}
\label{eqa:20}
\end{equation}

Figures~\ref{fig1-e} and~\ref{fig1-f} provide an intuitive demonstration of the trends in the divergence factor and the resulting weights: 
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item During the initial stages of training (e.g., prior to 700 steps), the slow decay of the divergence factor allows the relative convergence scores to predominate, resulting in Task B receiving the highest weight.
    \item As the convergence slope of Task B approaches zero swiftly, the divergence factor decays rapidly, leading to the dominance of the absolute convergence scores. Our method accurately captures the trend where the convergence slope of Task B begins to oscillate around zero, assigning it a smaller absolute convergence score. After 700 steps, the weight allocated to Task B rapidly decreases, effectively suppressing divergence.
\end{itemize}
\end{comment}


\paragraph{Difference from Exsiting Methods:}~Current approaches to convergence balancing, such as GradNorm~\cite{chen2018gradnorm}, IBTW~\cite{liu2019loss}, FAMO~\cite{liu2024famo}, and MetaWeighting~\cite{mao2022metaweighting}, are designed around the first criterion \textbf{\textit{c1}} outlined at the beginning of this section: decelerating the convergence of rapidly converging tasks while accelerating the convergence of slower tasks. The proposed RCS also accomplishes this objective effectively. Yet, it should be noted that this first criterion often has a counteractive effect on convergence balancing when certain tasks start to diverge. This is an issue that existing methods fail to address. To counteract this, CoBa introduces the ABS, which assigns lower weights to tasks that are diverging. Furthermore, DF improves this by detecting the divergence trend of tasks and subsequently magnifying the importance of ABS. This suppresses premature divergence trends, ensuring overall stability is maintained.

\begin{algorithm}[t]
    \caption{CoBa}
    \label{algo:1}
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \begin{algorithmic}[1]\small
        \REQUIRE Initial parameter $\theta_{0}$, $M$ batches of validation set, history window length $N=5M$, warm-up steps $W=M$, task number $K$, $\omega_{i}(0)=1/K$, validation loss ratios window $\vy_{i}(N;0) \leftarrow []$
        \ENSURE Trained parameter $\theta$
        \FOR{$t=0:T$}
            % \STATE Input training batch $\vx_{i}$ to compute $\ell_i(\theta;t)$ and $\ell(\theta;t) = \mathop{\sum}_{i=1}^{K}{\omega_{i}(t) \ell_i(\theta;t)}$
            \STATE Compute $\ell(\theta;t)$ with training batch $\vx_{t}$
            \STATE Compute $\Bar{\ell}_i^{val}(\theta;t)$ with validation batch $\vv_{t}$
            \STATE $\vy_{i}(N;t) \leftarrow [\Bar{\ell}_i^{val}(\theta;s_0),...,\Bar{\ell}_i^{val}(\theta;t)]^\top$
            \STATE Compute $\alpha_{i}(t)$ with (\ref{eqa:6}),(\ref{eqa:7})
            \IF{$t \le W$}
                \STATE Compute $RCS(t)$ with (\ref{eqa:RCS})
                \STATE Compute $ACS(t)$ with (\ref{eqa:ACS})
                \STATE Compute $DF(t)$ with (\ref{eqa:16})
                \STATE Compute $\omega(t)$ with (\ref{eqa:19})
            \ELSE
                \STATE Compute $\omega_{i}(t) = \frac{1}{K}$
            \ENDIF
        \ENDFOR
    \end{algorithmic}
\vspace{-0.3ex}
\end{algorithm}

\subsection{Complexity Analysis}
The overall algorithm is summarized in Algorithm~\ref{algo:1}. Here, we provide an analysis of CoBa's computational complexity. For our assumptions, we assign the computational complexity of forward propagation as $F$ and the complexity of backward propagation as $B$. We denote the number of tasks as $K$, the length of the history window as $N$, and the number of training iterations as $T$. Initially, CoBa calculates the loss for a training batch which updates the parameters, and this process costs $\gO(F+B)$ time. Subsequently, it evaluates the validation batch's loss, taking $\gO(F)$ time. Then, it calculates the convergence slopes $\valpha(t) = [\alpha_1(t),\cdots,\alpha_K(t)]^\top$ which requires $\gO(2KN)$ flops. The computation of $\RCS(t)$ and $\ACS(t)$ costs $\gO(5K)$ and $\gO(3K+2N)$ time, respectively. Ultimately, the identification of $\DF(t)$ and weight consumes $\gO(7T)$ and $\gO(3K)$ time, respectively. Thus, the joint time complexity of CoBa is $\gO(2F+B+2KN+11K+2N+7T)$. In terms of $F$, $B$, and $K$, this expression can be simplified to $\gO(a_3 F+a_2 B+a_5 K)$, as shown in Table~\ref{tab:time-complexity}.


%We assume $F$ is the computational complexity of the forward propagation, $B$ is the complexity of backward propagation, $K$ refers to the number of tasks, $N$ refers to length of history window, and $T$ refers to number of training iterations. First, CoBa computes the loss for a training batch and updates parameters, which cost $O(F+B)$ time. Second, the loss for a validation batch is evaluated, requiring $O(F)$ time. Third, the computation of the convergence slopes $\valpha(t) = [\alpha_1(t),\cdots,\alpha_K(t)]^\top$ requires $O(2KN)$ flops. Fourth, calculating $\RCS(t)$ and $\ACS(t)$ demands $O(5K)$ and $O(3K+2N)$ time, respectively. Finally, the determination of $\DF(t)$ and weight consume $O(7T)$ and $O(3K)$ time, respectively. Hence, the aggregate time complexity of CoBa can be expressed as $O(2F+B+2KN+11K+2N+7T)$. In terms of $F$, $B$, and $K$, the expression can be simplified as $O(a_3 F+a_2 B+a_5 K)$, as shown in Table~\ref{tab:time-complexity}. 
% 


==> contents/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

% Existing multi-task learning methods aim to address the issue of task imbalance and can broadly be categorized into two types: those based on task loss balance and those based on task gradient balance. Task loss balancing techniques dynamically adjust the weights assigned to each task throughout the training process based on heuristic methods, such as task uncertainty~\cite{kendall2018multi}, gradient normalization~\cite{chen2018gradnorm}, task difficulty prioritization~\cite{guo2018dynamic}, weight average~\cite{liu2019end} and random loss weighting~\cite{lin2021closer}. Despite their merits, such heuristic studies are susceptible to performance instability when task conflicts occurring.
% % Despite their merits, such studies obviously overlooking the convergence balance of validation losses, focusing on training losses solely. 
% % Besides, the task gradient balancing techniques 
% Another type of methods try to alleviate task conflicts by meticulously calibrating the gradients attributed to each task. A representative work applies a multiple-gradient descent algorithm (MGDA) to refine multi-task learning~\cite{desideri2012multiple}. Nevertheless, both categories of methods focus solely on training losses, consequently overlooking the critical gap between training and validation losses.

% To this end, a study~\cite{jean2019adaptive} utilizes validation BLEU scores to control task weight for multilingual machine translation. Recently, MetaWeighting~\cite{mao2022metaweighting} underline the gap between training and validation losses, and try to find task weights that narrow this gap based on meta-learning.

% The effectiveness of these strategies has been validated on small-scale models and simple classification tasks. Yet, the considerable computational demands and challenges in implementation within parallel training frameworks have hindered their application in training the latest LLMs. To explore the application of generative tasks and large models in multi-task learning, some frameworks such as Muppet~\cite{aghajanyan2021muppet} and ExT5~\cite{aribandi2021ext5} have emerged, further advancing research in this direction.

% Notwithstanding the contributions of the aforementioned methods, they neglect the issue of task convergence imbalance: diverging and converging tasks are simultaneously present during the training phase. This imbalance potentially produces overfitting on the validation data for some tasks, thereby deteriorating their performance. Unlike these methods, the approach proposed in this paper is designed to attain a state of convergence balance. It mitigates the tendency for early divergence of particular tasks, thereby substantively augmenting the overall performance. Additionally, the proposed method  is readily integrable into prevailing parallel training architectures, facilitating economical multi-task training for LLMs.

\begin{comment}
\subsection{MTL Methods for Task Balancing}
Existing multi-task learning (MTL) methods designed to address the issue of task imbalance can be broadly categorized into two types: task loss balancing methods and task gradient balancing methods. Task loss balancing methods dynamically adjust the weight of each task during training based on various heuristic approaches, such as task uncertainty~\cite{kendall2018multi}, gradient normalization~\cite{chen2018gradnorm}, task difficulty prioritization~\cite{guo2018dynamic}, weight average~\cite{liu2019end} and random loss weighting~\cite{lin2021closer}. However, these heuristic methods are prone to instability in performance when task conflicts occur. In contrast, task gradient balancing methods aim to mitigate task conflicts by adjusting the gradients of each task. For instance, Désidéri et al. leverage the Multiple Gradient Descent Algorithm (MGDA)~\cite{desideri2012multiple} to optimize MTL tasks. Similarly, Mao et al. propose the MetaWeighting~\cite{mao2022metaweighting}, which underline the gap between training and validation losses, and try to find task weights that narrow this gap based on meta-learning. 

Although the effectiveness of these methods has been validated in small-scale models and simple classification tasks, they face significant challenges when applied to the training of advanced LLMs. These challenges can be summarized as follows:
\begin{itemize}[leftmargin=*, topsep=1pt,itemsep=1pt,partopsep=1pt,parsep=1pt]
    \item High Computational Complexity: These methods often have high computational overhead, which can slow down training processes. For instance, FAMO~\cite{liu2024famo} and MetaWeighting~\cite{mao2022metaweighting} require at least two rounds of forward and backward propagation per iteration.
    \item Incompatibility with Training Acceleration Strategies: Due to training acceleration strategies such as ZeRO~\cite{rajbhandari2020zero} and Fully Sharded Data Parallel (FSDP)~\cite{zhao2023pytorch}, which partition model gradients, these methods struggle to adapt to mainstream parallel training frameworks when manipulating gradients.
    \item Suboptimal Performance with Small Learning Rates: LLMs training typically employs smaller learning rates, which can hinder these methods from achieving optimal results, such as GradNorm~\cite{chen2018gradnorm}.
\end{itemize}

\subsection{MTL Methods for LLMs}
In the realm of LLMs, parameter sharing is particularly crucial. Not only does it save computational and storage resources, but it also allows LLMs to utilize a shared set of parameters to handle multiple related tasks effectively. In recent years, substantial advances have been made in applying MTL techniques to LLMs. Raffel et al. introduce the T5~\cite{raffel2020exploring}, which explores the application of MTL techniques in more challenging generative tasks within an encoder-decoder architecture. Subsequently, Aghajanyan et al. propose Muppet~\cite{aghajanyan2021muppet}, which implements MTL between the pre-training and fine-tuning stages, termed as pre-fine-tuning (PFT). They find that incorporating this additional stage enhances the performance of pre-trained models on various downstream tasks and significantly speeds up fine-tuning. Building on T5, Aribandi et al. extend the methodology to ExT5~\cite{aribandi2021ext5}, increasing the number of tasks to 107 and further enhancing the multi-task performance.

Despite these promising results, these methods have not addressed the issue of task imbalance in MTL, especially the imbalance in convergence speed. Convergence speed imbalance is a phenomenon where the training trajectories of different tasks diverge: some tasks continue to converge on the validation set (underfitting), while others start to diverge (overfitting), ultimately degrading the performance on downstream tasks.

To better facilitate MTL in LLMs, this paper proposes a computationally simple yet effective MTL method that specifically addresses the issue of convergence imbalance across multiple tasks. 
\end{comment}

All Multi-Task Learning (MTL) approaches~\cite{crawshaw2020multi,vandenhende2021multi,zhang2023survey} are designed to foster positive knowledge transfer across tasks through parameter sharing, while simultaneously minimising any potential negative transfer, often referred to as task interference. Our discussion here primarily revolves around optimization techniques within MTL, given their relevance to LLMs. We categorize the existing work into two distinct groups: classical MTL methods and MTL methods tailored for LLMs.

\vspace{-1ex}
\paragraph{Classical Methods}
Traditional MTL strategies aimed at addressing task imbalance from an optimization standpoint fall into two categories: gradient manipulation and loss balance. Gradient manipulation techniques~\cite{chen2020just,liu2020towards,yu2020gradient,liu2021conflict} create a composite update vector at each optimization step by amalgamating task gradients. This approach ensures local improvements across all tasks but can be computationally intensive, particularly for models with numerous parameters. Conversely, loss balancing methods dynamically adjust each task's weight during training based on predefined factors such as task uncertainty~\cite{kendall2018multi}, task difficulty prioritization~\cite{guo2018dynamic}, and random loss weighting~\cite{lin2021closer}. These methods are computationally more efficient but do not guarantee simultaneous convergence of all tasks. To overcome this issue, advanced solutions aiming at convergence balance include DWA~\cite{liu2019end}, LBTW~\cite{liu2019loss}, GradNorm~\cite{chen2018gradnorm},  MetaWeighting~\cite{mao2022metaweighting}, and FAMO~\cite{liu2024famo}. The latter three adjust task weights based on gradients, with MetaWeighting additionally focusing on the validation instead of the training loss to enhance generalization performance. Unfortunately, gradient-based weight adjustment can be computationally demanding, as shown in Table~\ref{tab:time-complexity}. %, and may not integrate well with parallel training architectures like Deepspeed and FSDP, which could partition gradients.

\vspace{-1ex}
\paragraph{Methods for LLMs}
MTL research specific to LLMs is still in its infancy, with a handful of notable contributions from models such as T5~\cite{raffel2020exploring}, Muppet~\cite{aghajanyan2021muppet}, ExT5~\cite{aribandi2021ext5}, and MFTcoder~\cite{liu2023mftcoder}. The initial three primarily aggregate data from various tasks without considering task equilibrium, often overlooking tasks with smaller datasets and favoring those with larger ones. MFTcoder advances this by calculating individual loss for each task, yet assigns equal weights across the board. MFTcoder acknowledges the inability of such approaches to ensure uniform validation loss convergence across tasks and suggests leveraging FAMO as a potential solution.

The proposed method, CoBa, embodies the strengths of both classical and LLM-specific MTL approaches, achieving convergence balance among tasks with minimal additional computational demands. Crucially, it focuses on validation loss, thereby promising to maintain or improve the generalization capabilities of the model.
